Camera Calibration and Player Localization in SoccerNet-v2 and Investigation of their Representations for Action Spotting

Soccer broadcast video understanding has been drawing a lot of attention in recent years within data scientists and industrial companies. This is mainly due to the lucrative potential unlocked by effective deep learning techniques developed in the field of computer vision. In this work, we focus on the topic of camera calibration and on its current limitations for the scientific community. More precisely, we tackle the absence of a large-scale calibration dataset and of a public calibration network trained on such a dataset. Specifically, we distill a powerful commercial calibration tool in a recent neural network architecture on the large-scale SoccerNet dataset, composed of untrimmed broadcast videos of 500 soccer games. We further release our distilled network, and leverage it to provide 3 ways of representing the calibration results along with player localization. Finally, we exploit those representations within the current best architecture for the action spotting task of SoccerNet-v2, and achieve new state-of-the-art performances.

==> sections/5_discussion.tex <==
\section{Discussion}

Blaaaa.

==> sections/old-plan.tex <==
\begin{itemize}
    \item We use a private commercial calibration tool (name EVS if you want, that would be a free advertisement) to obtain calibrations on the SoccerNet train set.
    \item The commercial tool cannot be released.
    \item We use these annotations as surrogate ground truths to train a lightweight and faster student network (distillation).
    \item The student is inspired from the CVPR2020 paper~\cite{Sha2020End}. There are some minor modifications (explain them briefly). No need to explain the whole network architecture nor functioning, as it is not our work.
    \item We use the student rather than the teacher because we want to allow reproducibility of our experiments and usage of our pipeline outside soccernet, which would not be possible with the private teacher.
    \item Hence, we release the student.
    \item Note: given the performances of the student: it's just good enough to be used legitimately rather than existing available calibration tools, and it's bad enough to avoid releasing a tool with a commercial value. Thus, good for research, not for industries.
    \item We report the performances of the teacher to validate its use as teacher (and for EVS, free advertisement). Those performances also allow to show that the distillation loses some performance, but not too much.
    \item We can say that the teacher will be released in a future paper with all the details (if you want).
\end{itemize}

\subsection{Action spotting}

\begin{itemize}
    \item We investigate how to use the calibration to improve the action spotting on SoccerNet-v2.
    \item We compute a top view of the field with the players on it.
    \item We feed that to our great network (described in detail)
    \item We have super performances.
    \item We investigate graph neural networks with players positions in it... still bad at the moment.
\end{itemize}

\subsection{Contributions}

\begin{itemize}
    \item In this paper, our contributions are the following.
    \item We release a fast lightweight calibration tool, distilled from a SOTA commercial tool.
    \item We include the calibration information for the task of action spotting in different ways and show why it is useful.
    \item We have awesome results on action spotting that can be reproduced and exported on other matches (well, maybe, if they are good enough, as always).
\end{itemize}
